Contextual Bandits with Budgeted Information Reveal

Contextual bandit algorithms are commonly used in digital health to recommend personalized treatments. However, to ensure the effectiveness of the treatments, patients are often requested to take actions that have no immediate benefit to them, which we refer to as pro-treatment actions. In practice, clinicians have a limited budget to encourage patients to take these actions and collect additional information. We introduce a novel optimization and learning algorithm to address this problem. This algorithm effectively combines the strengths of two algorithmic approaches in a seamless manner, including 1) an online primal-dual algorithm for deciding the optimal timing to reach out to patients, and 2) a contextual bandit learning algorithm to deliver personalized treatment to the patient. We prove that this algorithm admits a sub-linear regret bound. We illustrate the usefulness of this algorithm on both synthetic and real-world data.

==> thompson_sampling.tex <==
\section{Attempt for Thompson Sampling}
\begin{algorithm}
\caption{Online Learning Algorithm}
\label{alg:learning-reward}
\begin{algorithmic}
\State \textbf{Input:} $B, \mathbf{p}_k$
\State \textbf{Initialize:}
$\hat \mu^1$ and $\hat \Sigma^1$ as the mean and covariance matrix of the Gaussian prior over $\theta_*$ for the treatment recommender, respectively; $\tilde \mu^1$ and $\tilde \Sigma^1$ as the mean and covariance matrix of the Gaussian prior over $\theta_*$ for the information revealer, respectively.
\For{$t=1,...,T$}
\State On each day $t$, the information revealer observes the new context $s_t$.
\State The information revealer samples $\Tilde{\theta}(t) \sim \mathcal{N}(\tilde \mu^t,(\tilde \Sigma^t)^{-1})$.
\State The treatment recommender samples $\hat {\theta}(t)\sim \mathcal{N}(\hat \mu^t,(\hat \Sigma^t)^{-1})$.
\State Calculate $\tilde a_t = \argmax_{a\in \mathcal{A}}\left\langle\tilde{\theta}(t), \phi(s_t, a)\right\rangle$ and $\hat a_t = \argmax_{a\in \mathcal{A}}\left\langle\hat{\theta}(t), \phi(s_t, a)\right\rangle$.
\State Calculate $\Tilde{u}_{s_t}^t =  \langle \Tilde{\theta}(t), \phi(s_t, \tilde a_t)\rangle$, 
$\Tilde{v}^t = \left\langle\Tilde{\theta}(t), 
\bar\phi(\tilde a_t)
\right\rangle$, and 
$\bar{v}^t = \left\langle\tilde{\theta}(t), 
\bar\phi(\hat a_t)
\right\rangle$.
\State Given $\Tilde{u}_{s_t}^t$, $\Tilde{v}^t$, $\bar{v}^t$, $\tilde a_t$, and $\hat a_t$, the information revealer uses Algorithm~\ref{alg:primal-dual-step-constraint} to reveal $\mathcal{H}_{t}^{\mathrm{ir}}$ to the treatment recommender with probability: $O_t = \mathrm{Bernoulli}(o_t)$.
\If{$O_t=1$}
\State Set $\hat \Sigma^{t} = \tilde \Sigma^{t}$ and $\hat \mu^{t} = \tilde \mu^{t}$.
\State Choose the action $a_t^* = \argmax_{a\in \mathcal{A}}\left\langle\Tilde{\theta}(t), \phi(s_t, a)\right\rangle$.
\State Observe the realized reward $x_t$, and update
% \State Observe additional realized rewards $x_{w}, ..., x_{t-1}$.
% \State Set 
% 
\begin{align*}
% $$
\tilde \Sigma^{t+1} &=
 \tilde \Sigma^{t} + \phi(s_{t}, a^*_{t}) \; \phi(s_{t}, a^*_{t})^\top, \\
 g^{t+1} &= g^{t} + x_t\phi(s_{t},a_{t}^*),\\ 
 \tilde \mu^{t+1} &= \left(\tilde\Sigma^{t+1}\right)^{-1} g^{t+1}.
 % +\sum_{i=w}^{t-1} x_i \; \bar{\phi}(a_i)\bar{\phi}(a_i)^T
 % + 
 % \sum_{i=w}^{t-1}\bar{\phi}(a_i)\bar{\phi}(a_i)^T.
 % $$
 % \\
% &  \sum_{i=v}^{t-1}\left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right) \left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right)^\top.
\end{align*}
% \State Set $g^{t+1} = g^{w} + x_w\phi(s_{w-1},a_{w-1}^*) +\sum_{i=w}^{t-1} x_i \; \bar{\phi}(a_i)\bar{\phi}(a_i)^T
% % \left(\sum_{k=1}^K \phi(S_t=k, a^*_i)p(S_t=k)\right)
% .$
% \State Set $u^{t+1} = \left(\Sigma^{t+1}\right)^{-1} g^{t+1}.$
% \State $w\leftarrow t+1$.
% \State Sample $\Tilde{\theta}(t)$ from the posterior distribution $\mathcal{N}(u^{t+1},(\Sigma^{t+1})^{-1})$.
\Else 
\State Choose the action $a_t^* = \argmax_{a \in \mathcal{A}} \left\langle\hat{\theta}(t), 
\bar{\phi}(a)
% \sum_{k=1}^K\phi(S_t=k, a) p(S_t=k)
\right\rangle
$.
\State Observe the realized reward $x_t$ and update
\begin{align*}
% $$
\tilde \Sigma^{t+1} &=
 \tilde \Sigma^{t} + \bar\phi(a^*_{t}) \; \bar\phi(a^*_{t})^\top, \\
 g^{t+1} &= g^{t} + x_t\bar\phi(a_{t}^*),\\ 
 \tilde \mu^{t+1} &= \left(\tilde\Sigma^{t+1}\right)^{-1} g^{t+1}.
 % +\sum_{i=w}^{t-1} x_i \; \bar{\phi}(a_i)\bar{\phi}(a_i)^T
 % + 
 % \sum_{i=w}^{t-1}\bar{\phi}(a_i)\bar{\phi}(a_i)^T.
 % $$
 % \\
% &  \sum_{i=v}^{t-1}\left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right) \left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right)^\top.
\end{align*}
\State Set $\hat \Sigma^{t+1} = \hat \Sigma^{t}$ and $\hat \mu^{t+1} = \hat \mu^t$.
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
% \begin{algorithm}
% \caption{Online Learning Algorithm}
% \label{alg:learning-reward}
% \begin{algorithmic}
% \State \textbf{Input:} $B, p(S_t = k)$
% % \State \textbf{Input:} $B, \{u_{s_t}^*\}_{s_t\in S}, v^*, c= (1+1/B)^B$
% \State \textbf{Initialize:}
% $u^1$ and $\Sigma^1$ as the mean and covariance matrix of the Gaussian prior over $\theta_*$, respectively; $v\leftarrow 1$.
% \For{$t=1,...,T$}
% \State On each day $t$, the second agent observes the new context $s_t$.
% \State Sample $\Tilde{\theta}(t)$ from the posterior distribution $\mathcal{N}(u^t,(\Sigma^t)^{-1})$.
% \State Set $\Tilde{u}_{s_t}(t) = \max_{a\in \mathcal{A}} \langle \Tilde{\theta}(t), \phi(s_t, a)\rangle$ and $\Tilde{v}(t) = \max_{a\in \mathcal{A}}\left\langle\Tilde{\theta}(t), \sum_{k=1}^K\phi(S_t=k, a) p(S_t=k)\right\rangle$.
% \State Given the estimated $\Tilde{u}_{s_t}(t)$ and $\Tilde{v}(t)$, the second agent uses Algorithm~\ref{alg:primal-dual-step-constraint} to reveal the current context to the first agent with probability: $O_t = \mathrm{Bernoulli}(o_t)$.
% \If{$O_t=1$}
% \State Observe additional realized rewards $x_{v}, ..., x_{t-1}$.
% \State Choose the action $a_t^* = \argmax_{a\in \mathcal{A}}\left\langle\Tilde{\theta}(t), \phi(s_t, a)\right\rangle$.
% \State Set 
% % \begin{align*}
% $$\Sigma^{t+1} =
% % &
%  \Sigma^{v} + \phi(s_{v-1}, a^*_{v-1}) \; \phi(s_{v-1}, a^*_{v-1})^\top + 
%  \sum_{i=v}^{t-1}\bar{\phi}(a_i)\bar{\phi}(a_i)^T.$$
%  % \\
% % &  \sum_{i=v}^{t-1}\left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right) \left( \sum_{k=1}^K\phi(S_t=k, a^*_i)p(S_t=k)\right)^\top.
% % \end{align*}
% \State Set $g^{t+1} = g^{v} + x_v\phi(s_{v-1},a_{v-1}^*) +\sum_{i=v}^{t-1} x_i \; \bar{\phi}(a_i)\bar{\phi}(a_i)^T
% % \left(\sum_{k=1}^K \phi(S_t=k, a^*_i)p(S_t=k)\right)
% .$
% \State Set $u^{t+1} = \left(\Sigma^{t+1}\right)^{-1} g^{t+1}.$
% \State $v\leftarrow t+1$.
% \Else 
% \State Choose the action $a_t^* = \argmax_{a \in \mathcal{A}} \left\langle\Tilde{\theta}(t), 
% \bar{\phi}(a)
% % \sum_{k=1}^K\phi(S_t=k, a) p(S_t=k)
% \right\rangle
% $.
% \State $\Sigma^{t+1} = \Sigma^{t}$.
% \State $u^{t+1} = u^t$.
% \EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}



% \kyra
% {To be fixed later:
 

% Before we prove Proposition~\ref{thm:bandit_learning}, we first want to show the concentration of $\hat \theta_t$ at the steps when we reveal the context, where $\hat\theta_t$ is the solution of the least-square estimator, we will rigorously define $\hat\theta_t$ in Proposition~\ref{prop:concentration}.

\newpage
\begin{prop}\label{prop:concentration} Assume that $\|\theta_*\|_2 \leq S$ with Q-probability one and $\sup_{a\in \mathcal{A}, s_t\in S}\|\phi(s_t,a)\|\leq L$ and $\sup_{a\in \mathcal{A}, s_t\in S}\langle\phi(s_t,a),\theta_*\rangle \leq 1$ with Q-probability one. Let $\hat\theta_t$ be the $L^2$-regularised least-square estimator for $\theta_*$, and 
let $\delta\in(0,1)$.
Then, with probability at least $1-\delta$, the following inequality holds for any $t\in [T]$ and
$\lambda>0$:
% and $\delta\in(0,1)$, 
$$\left\|\theta_* - \hat\theta_t\right\|_{V_t(\lambda)}\leq \sqrt{2\log\left(\frac{1}{\delta}\right) + \log\left(\frac{\det(\tilde V_t(\lambda))}{\lambda^q}\right)} + \sqrt{\lambda}\norm{\theta_*}_2 + c,
$$
where $c=\Bigg\| 
\sum_{i=\ell(t)}^{t-1} \phi(s_i, a_i)O_i+ \sum_{i=\ell(t)}^{t-1} \bar{\phi}(a_i)(1-O_i) 
\Bigg\|_{V_t(\lambda)^{-1}}.$
% it holds that for all $t$ where $O_t=1$,
% $$\|\hat\theta_t - \theta_*\|_{V_t(\lambda)}<...$$
\end{prop}

\begin{proof}[Proof of Proposition~\ref{prop:concentration}]
Let $$\phi_t(A_t) := \phi(S_t, A_t)O_t+\bar\phi(A_t)(1-O_t).$$ 
Recall that we assumed $X_{t} (S_t, A_t)$ as the uncertain reward feedback of patient $t$ with context $S_t$ assigned to action $A_t$:
$$ X_{t} (S_t, A_t) = \langle \theta_*, \phi(s_t, a_t)\rangle O_t + \langle \theta_*, \bar{\phi}(a_t)\rangle (1-O_t) +
\eta_t = \langle \theta_*, \phi_t(a_t)\rangle +
\eta_t .$$
If we were to observe the realized reward up to time $t$ (noninclusive) at each step, 
the $L^2$-regularised least-square estimator of $\theta_*$ at time $t$, $\tilde \theta_t$, can be obtained by solving the following optimization problem:
\begin{align*}
L_t(\theta) &= \lambda \|\theta\|^2 + \sum_{i=1}^{t-1}
% \left(\left( X_i -\langle \theta, \phi(s_i, a_i)\rangle  \right)^{2} O_i +  \left( X_i -\langle \theta, \bar{\phi}(a_i)\rangle  \right)^{2}  (1-O_i)\right)
\left(\left( X_i - \left\langle \theta, \phi(s_i, a_i)O_i + \bar{\phi}(a_i)(1-O_i)\right\rangle  \right)^{2} \right) 
\\& =
\lambda \|\theta\|^2 + \sum_{i=1}^{t-1}\left(\left( X_i - \left\langle \theta, \phi_i(a_i)\right\rangle  \right)^{2} \right) ,
\end{align*}
where $\lambda > 0$ is the regularization parameter. 


Minimizing the above term ($\nabla_\theta {L}_{t}(\theta) = 0$) yields the following estimator for $\theta_*$:
\begin{align*}
\tilde{\theta}_t &= 
\left (  
\sum_{i=1}^{t-1} \phi_i(a_i)\phi_i(a_i)^T 
% + \sum_{i=1}^{t-1} \bar{\phi}(a_i)\bar{\phi}(a_i)^T(1-O_i)
+ \lambda I
\right )^{-1}  
% \\ &\quad \quad \quad \quad 
\left (  
\sum_{i=1}^{t-1} \phi_i(a_i)X_i
\right ).
\end{align*} 


Note that $\tilde\theta_t$ implicitly assumes that at each step, we observe the rewards of the actions that we have taken up to time $t$.
However, since when the information revealer decides to not reveal, the treatment recommender gets no additional information, we can only use the information that is revealed to the treatment recommender prior to (noninclusive) the most recent reveal. 
At time $t$, let $\ell(t)$ denote the most recent time that we reveal $\mathcal{H}^{\mathrm{ir}}_{\ell(t)}$ to the treatment recommender. Then by time $t$, we observe  rewards $X_1, ..., X_{\ell(t)-1}$.
Then, the $L^2$-regularised least-square estimator of $\theta_*$ at time $t$, $\hat\theta_t$ as follows:
% 
% \esmaeil{When we estimate $\theta_{*}$ at time $t$, we need to incorporate all the {\em available} information up to the current time $t$ that we used in our posterior at the start of time $t$ in Algorithm 3. So, I was wondering if the time index $\ell(t)$ that you defined captures this issue? 
% 
% Another way we can develop this estimator is by defining the {\em information set} $\mathcal{I}_t$, which is the set of time-stamps with the context and rewards realized by time period $t$, i.e., $\left\{ X_i, \phi(s_i, a^*_i), \bar{\phi}(a_i) \right\}_{i = 1}^{\ell(t)-1}$.
% %$$
% %\mathcal{F}_t = \left\{ X_i, \phi(s_i, a^*_i), \bar{\phi}(a_i) \right\}_{i = 1}^{t-1}
% %$$
% %$$
% %\mathcal{F}_t = \left\{ \{X_i\}_{i = v}^{t-1}, %\phi(s_{v-1}, a^*_{v-1}), \bar{\phi}(a_i) \right\}
% %$$
% Then, the regularized least-square estimator at time $t$ is obtained as follows:
% \begin{align*}
% \hat{\theta}_t &= 
% \left (  
% \sum_{i \in \mathcal{I}_t} \phi(s_i, a_i)\phi(s_i, a_i)^TO_i+ \sum_{i \in \mathcal{I}_t} \bar{\phi}(a_i)\bar{\phi}(a_i)^T(1-O_i) + \lambda I
% \right )^{-1}  
% \\ &\quad \quad \quad \quad 
% \left (  
% \sum_{i \in \mathcal{I}_t} \phi(s_i, a_i)X_iO_i+ \sum_{i \in \mathcal{I}_t} \bar{\phi}(a_i)X_i(1-O_i) 
% \right ).
% \end{align*}
% So, just want to ensure that this estimator and the following you wrote are the same.}
% 
\begin{align*}
\hat{\theta}_t &= 
\left (  
\sum_{i=1}^{\ell(t)-1} \phi_i(a_i)\phi_i(a_i)^T
% + \sum_{i=1}^{\ell(t)-1} \bar{\phi}(a_i)\bar{\phi}(a_i)^T(1-O_i) 
+ \lambda I
\right )^{-1}  
% \\ &\quad \quad \quad \quad 
\left (  
\sum_{i=1}^{\ell(t)-1} \phi_i( a_i)X_i 
\right ).
\end{align*} 
Let $$V_t(\lambda) = \lambda I + \sum_{i=1}^{\ell(t)-1}  \phi_i(a_i) \phi_i(a_i)^T. 
$$ 
For notational convenience, we let $V_t:= V_t(0)$.  
% Let $\zeta_t(a_t):= \eta_t\phi_t(a_t).$
Then, $\hat\theta_t$ can be rewritten as  
\begin{align*}
\hat\theta_t &= V_t(\lambda)^{-1}\left ( \sum_{i=1}^{\ell(t)-1} \phi_i(a_i)X_i 
\right )
% \\&
=V_t(\lambda)^{-1}\left ( \sum_{i=1}^{\ell(t)-1} \phi_i(a_i)\left(\langle  \theta_*, \phi_i(a_i)\rangle +\eta_i \right)
\right )\\
&= V_t(\lambda)^{-1}\left ( 
V_t \theta_* +
\sum_{i=1}^{\ell(t)-1} 
 \phi_i(a_i)\eta_i 
\right ) 
% =  V_t(\lambda)^{-1}\left ( 
% V_t \theta_* +
% \sum_{i=1}^{\ell(t)-1} 
% \phi_i(a_i)\eta_i(a_i)
% \right )
.
\end{align*}
% \esmaeil{(Note for myself) Basically, $\sum_{i=1}^{\ell(t)-1} 
% \phi_i(a_i)\eta_i$ is the martingale which is critical in the analysis, and we need to separate it from the design matrix $\tilde V_t(\lambda)$ later on.}

Similarly, let 
$$\tilde V_t(\lambda) = \lambda I + \sum_{i=1}^{t-1}\phi_i(a_i) \phi_i(a_i)^T,$$ and let $\tilde V_t = V_t(0)$, then we can rewrite $$\tilde \theta_t = {\tilde V_t(\lambda)}^{-1}\left ( 
\tilde V_t \theta_* +
\sum_{i=1}^{t-1} 
 \phi_i(a_i)\eta_i
\right ).$$
% $\tilde \theta_t = {\tilde V_t(\lambda)}^{-1}\left ( 
% \tilde V_t \theta_* +
% \sum_{i=1}^{t-1} 
%  \phi(s_i, a_i)\eta_iO_i+
% \sum_{i=1}^{t-1}  \bar\phi(a_i)\eta_i(1-O_i)
% \right ).$


Use the following decomposition:
$\theta_*- \hat{\theta}_t = \left ( \theta_*-\tilde {\theta}_t  \right ) + \left ( \tilde{\theta}_t-\hat{\theta}_t \right ), $
next, we derive the upper bound for $\left\langle\theta_* - \hat\theta_t, \phi_t(a_t)
\right\rangle$
by applying the triangle inequality:
\begin{align*}
\left|\left\langle\theta_* - \hat\theta_t, \phi_t(a_t)
\right\rangle\right|
% \left\|\theta_* - \hat\theta_t\right\|_{V_t(\lambda)}
&\leq 
\underbrace{ 
\left|\left\langle\theta_* - \tilde\theta_t, \phi_t(a_t)
\right\rangle\right|
% \left\|\theta_* - \tilde\theta_t\right\|_{\tilde V_t(\lambda)}
}_{\text{(I)}}
+\underbrace{ 
\left|\left\langle\tilde\theta_t - \hat\theta_t, \phi_t(a_t)
\right\rangle\right|
% \left\|\tilde\theta_t - \hat\theta_t\right\|_{V_t(\lambda)}
}_\text{(II)}.
\end{align*}
% The last inequality is due to the observation that 
% $\tilde V_t(\lambda) \preceq V_t(\lambda)$. We note that 
% if $A \preceq B$, then $\norm{x}_A \leq \norm{x}_B$ for any vector $x$.


Next, we bound the above two terms separately:

\paragraph{Term (I):} 
We first note that by Cauchy–Schwarz inequality, we have
\begin{align*}
    \left\lvert \left\langle\, \theta_* - \tilde \theta_t, \phi_t(a_t)\right\rangle \right\rvert     
    % &=\left|\left\langle
%     {\tilde V_t(\lambda)}^{-1} 
% \left(
% \sum_{i=1}^{t-1} \phi_i(a_i)\eta_i
% \right) +
% \left(\tilde V_t(\lambda)^{-1}\tilde V_t-I\right)\theta_*, 
% \phi_t
% \right\rangle\right|
    % \\&
\leq \left\|\phi_t(a_t)\right\|_{{\tilde V_t(\lambda)}^{-1}} \left\|\theta_* - \tilde \theta_t \right\|_{\tilde V_t(\lambda)}.
\end{align*}
Following the proof of Theorem 20.5 in 
\cite{lattimore2020bandit}, we can show that the following holds for any $t$:
\begin{align*}
&\left\|\theta_* - \tilde\theta_t\right\|_{\tilde V_t(\lambda)} = 
\left\|{\tilde V_t(\lambda)}^{-1} 
\left(
\sum_{i=1}^{t-1} \phi_i(a_i)\eta_i
\right) +
\left(\tilde V_t(\lambda)^{-1}\tilde V_t-I\right)\theta_*
\right\|_{\tilde V_t(\lambda)}\\
&\leq \left\|{\tilde V_t(\lambda)}^{-1} 
\left(
\sum_{i=1}^{t-1} \phi_i(a_i)\eta_i
\right) 
\right\|_{\tilde V_t(\lambda)} 
+
\left\|
\left(\tilde V_t(\lambda)^{-1}\tilde V_t-I\right)\theta_*
\right\|_{\tilde V_t(\lambda)}\\
&= \left\|\sum_{i=1}^{t-1} 
\phi_i(a_i)\eta_i
\right\|_{\tilde V_t(\lambda)^{-1}} + 
\sqrt{\theta_*^\top (\tilde V_t(\lambda)^{-1}\tilde V_t-I)\tilde V_t(\lambda)(\tilde V_t(\lambda)^{-1}\tilde V_t-I)\theta_*
}\\ 
&= \left\|\sum_{i=1}^{t-1} 
\phi_i(a_i)\eta_i
\right\|_{\tilde V_t(\lambda)^{-1}} +
\sqrt{\lambda}\sqrt{\theta_*^\top(I-\tilde V_t(\lambda)^{-1}\tilde V_t)\theta_*}
 \;\leq \;\left\|\sum_{i=1}^{t-1} 
\phi_i(a_i)\eta_i
\right\|_{\tilde V_t(\lambda)^{-1}} + \sqrt{\lambda}\norm{\theta_*}_2 
\end{align*}
where $\tilde V_t$ is the design matrix defined above and note that $\tilde V_t = \tilde V_t(\lambda) - \lambda I$.

Let $q$ be the dimension of $\phi_t(a_t)$, and since under $\tilde \theta_t$ we would have observed the history of the rewards up to time $t-1$ and the history of states up to time $t$, we consider the $\sigma$-algebra $\mathcal{F}_t :=  \sigma\left(X_1, ..., X_{t-1}, \phi_1(A_1) , ..., \phi_t(A_{t})\right)$. 

% \esmaeil{I think the $\sigma$-algebra $\mathcal{F}_{t}$ should be defined as follows:
% $$
% \mathcal{F}_{t} :=  \sigma(X_1, ..., X_{\ell(t)-1}, O_1\phi(S_1, A_1) + (1-O_1)\bar\phi(A_1), ..., O_{t}\phi(S_{t}, A_{t}) + (1-O_t)\bar\phi(A_t))
% $$
% }

Recall that the noises $\eta_t$'s are conditionally 1-subgaussian: for all $\alpha \in \mathbb{R}$ and $t\geq 1$, $\mathbbm{E}\left[\exp(\alpha \eta_t)|\mathcal{F}_{t-1}\right]\leq \exp \left(\frac{\alpha^2}{2}\right) a.s.$ 
Then, following Lemmas 20.2 and 20.3, and Theorem 20.4 in \cite{lattimore2020bandit}, we have that for all $\lambda >0$ and $\delta \in (0,1)$:
$$\mathbbm{P}\left(\exists t\in \mathbbm{N}: \left\|\sum_{i=1}^{t-1} 
\phi_i(a_i)\eta_i
%  \phi(s_i, a_i)\eta_iO_i+
% \sum_{i=1}^{t-1}  \bar\phi(a_i)\eta_i(1-O_i)
\right\|_{\tilde V_t(\lambda)^{-1}}^2\geq 2\log(1/\delta) + \log(\det(\tilde V_t(\lambda))/\lambda^q)\right)\leq \delta.$$ 
Together, we have that
with probability $1-\delta$,
$$
\left\|\theta_* - \tilde \theta_t\right\|_{\tilde V_t(\lambda)} \leq 
\sqrt{2\log\left(\frac{1}{\delta}\right) + \log\left(\frac{\det(\tilde V_t(\lambda))}{\lambda^q}\right)} + \sqrt{\lambda}\norm{\theta_*}_2,
$$
and
\begin{align*}
    \left\lvert \left\langle\, \theta_* - \tilde \theta_t, \phi_t(a_t)\right\rangle \right\rvert     
\leq \left\|\phi_t(a_t)\right\|_{{\tilde V_t(\lambda)}^{-1}} 
\left(\sqrt{2\log\left(\frac{1}{\delta}\right) + \log\left(\frac{\det(\tilde V_t(\lambda))}{\lambda^q}\right)} + \sqrt{\lambda}\norm{\theta_*}_2\right).
% \left\|\theta_* - \tilde \theta_t \right\|_{\tilde V_t(\lambda)}.
\end{align*}

% Next, we want to show that the following holds:
% \begin{lemma}\label{lemma:supermartingale} For all $x\in \mathbb{R}^q$, the process $M_t(x) = \exp \Big(\Big\langle x, \Big\|\sum_{i=1}^{t-1} 
%  \phi(s_i, a_i)\eta_iO_i+
% \sum_{i=1}^{t-1}  \bar\phi(a_i)\eta_i(1-O_i)  \Big\|_{\tilde V_t(\lambda)^{-1}} \Big \rangle 
% -\frac{1}{2}\|x\|_{\tilde V_t(\lambda)}^2\Big)$ is an $\mathbb{F}$-adaptive and non-negative supermartingale with $M_0(x)\leq 1$.
% \end{lemma}
% \begin{proof}[Proof of Lemma~\ref{lemma:supermartingale}.]
    
% \end{proof}
\paragraph{Term (2)}: Since $\tilde V_t(\lambda)^{-1} \preceq V_t(\lambda)^{-1}$, we have that
\begin{align*}
    \left\lvert \left\langle\, \tilde\theta_t - \hat \theta_t, \phi_t(a_t)\right\rangle \right\rvert  
&=\left\lvert \left\langle
\tilde V_t(\lambda)^{-1}\left (  
\sum_{i=1}^{t-1} X_i \phi_i(a_t)
\right )  
-V_t(\lambda)^{-1}\left (  
\sum_{i=1}^{\ell(t)-1} X_i\phi_i(a_i) 
\right ), \phi_t(a_t)\right\rangle \right\rvert
\\&
\leq
\left\lvert \left\langle
V_t(\lambda)^{-1}\left (  
\sum_{i=\ell(t)}^{t-1} X_i \phi_i(a_t)
\right )  
, \phi_t(a_t)\right\rangle \right\rvert
\\& 
= \left\lvert \left\langle
V_t(\lambda)^{-1}\left ( X_{\ell(t)}\phi(s_{\ell(t)}, a_{\ell(t)}) + 
\sum_{i=\ell(t)+1}^{t-1} X_i \bar\phi(a_t)
\right )  
, \phi_t(a_t)\right\rangle \right\rvert,
\end{align*}
where the last equality is due to the fact that $O_i=0$ for $i\in[\ell(t)+1, t-1]$ by the definition of $\ell(t)$.
Our constraint implies that at any given time $t$, we have that $\left|\langle\tilde \theta_t - \hat \theta_t, \bar\phi(a_t)\rangle\right|(1-o_t) \leq \beta_t$.


\begin{align*}
&\left\|\tilde \theta_t - \hat\theta_t\right\|_{V_t(\lambda)}\\ 
&=
\Bigg\|\tilde V_t(\lambda)^{-1}\left (  
\sum_{i=1}^{t-1} X_i( \phi(s_i, a_i)O_i+ 
% \sum_{i=1}^{t-1} 
\bar{\phi}(a_i)(1-O_i))
\right )  
% \\
% & \quad \quad
-V_t(\lambda)^{-1}\left (  
\sum_{i=1}^{\ell(t)-1} X_i(\phi(s_i, a_i)O_i+ 
% \sum_{i=1}^{\ell(t)-1}
\bar{\phi}(a_i)(1-O_i) )
\right )
\Bigg\|_{V_t(\lambda)}\\
&
\leq \Bigg\|V_t(\lambda)^{-1}\left (  
\sum_{i=\ell(t)}^{t-1} \phi(s_i, a_i)X_iO_i+ \sum_{i=\ell(t)}^{t-1} \bar{\phi}(a_i)X_i(1-O_i) 
\right )
\Bigg\|_{V_t(\lambda)}\\
&=\Bigg\| 
\sum_{i=\ell(t)}^{t-1} X_i\left(\phi(s_i, a_i)O_i+  \bar{\phi}(a_i)(1-O_i) \right)
\Bigg\|_{V_t(\lambda)^{-1}}
% \\&
\leq \Bigg\| 
\sum_{i=\ell(t)}^{t-1}
\left(\phi(s_i, a_i)O_i+ 
% \sum_{i=\ell(t)}^{t-1} 
\bar{\phi}(a_i)(1-O_i) \right)
\Bigg\|_{V_t(\lambda)^{-1}}
% &=\left\| \left(\tilde V_t(\lambda)^{-1}\tilde V_t - V_t(\lambda)^{-1}V_t\right)\theta_* +
% {\tilde V_t(\lambda)}^{-1} 
% \left(\sum_{i=\ell(t)}^{t-1} 
% \phi_i(a_i)\eta_i
% \right) +
% (\tilde V_t(\lambda)^{-1} - V_t(\lambda)^{-1})\left(\sum_{i=1}^{\ell(t)-1}\phi_i(a_i)\eta_i\right)
% \right\|_{V_t(\lambda)}\\
% &\leq \left\|
% \left(\tilde V_t(\lambda)^{-1}\tilde V_t - V_t(\lambda)^{-1}V_t\right)\theta_* 
% \right\|_{V_t(\lambda)} + 
% \left\|
% {\tilde V_t(\lambda)}^{-1} 
% \left(\sum_{i=\ell(t)}^{t-1} 
% \phi_i(a_i)\eta_i
% \right)
% \right\|_{\tilde V_t(\lambda)} 
% \\
% &= \sqrt{\theta_*^\top(\left(V_t(\lambda)V_t - \tilde V_t(\lambda)^{-1}\tilde V_t\right)V_t + \left(\tilde V_t(\lambda)\tilde V_t - V_t(\lambda)^{-1}V_t\right)V_t(\lambda)\tilde V_t(\lambda)^{-1}\tilde V_t)\theta_*}
% + 
% \left\|\sum_{i=\ell(t)}^{t-1} \phi_i(a_i)\eta_i
% \right\|_{\tilde V_t(\lambda)^{-1}} 
% \\
% &\leq 
% \sqrt{\theta_*^\top\left(\tilde V_t(\lambda)^{-1}\tilde V_t - V_t(\lambda)^{-1}V_t\right)(\tilde V_t-V_t)\theta_*}
% % \left\|
% % \left(\tilde V_t(\lambda)^{-1}\tilde V_t - V_t(\lambda)^{-1}V_t\right)\theta_* 
% % \right\|_{V_t(\lambda)}
% % + 
% % \left\|\sum_{i=\ell(t)}^{t-1} 
% %  \phi(s_i, a_i)\eta_iO_i
% %  +
% % \sum_{i=\ell(t)}^{t-1}  \bar\phi(a_i)\eta_i(1-O_i)
% % \right\|_{\tilde V_t(\lambda)^{-1}}
% +\left\|\sum_{i=\ell(t)}^{t-1} \phi_i(a_i)\eta_i 
% \right\|_{\tilde V_t(\lambda)^{-1}} 
\end{align*}
We note that the first inequality holds because $\tilde V_t(\lambda)^{-1} \preceq V_t(\lambda)^{-1}$, and the last inequality holds because $X_i\in[-1,1]$ by our assumption.

Putting the two terms above together, we obtain that for $\lambda>0$ and $\delta\in(0,1)$, $$\left\|\theta_* - \hat\theta_t\right\|_{V_t(\lambda)}\leq \sqrt{2\log\left(\frac{1}{\delta}\right) + \log\left(\frac{\det(\tilde V_t(\lambda))}{\lambda^q}\right)} + \sqrt{\lambda}\norm{\theta_*}_2 + c,
$$
where $c=\Bigg\| 
\sum_{i=\ell(t)}^{t-1} \phi(s_i, a_i)O_i+ \sum_{i=\ell(t)}^{t-1} \bar{\phi}(a_i)(1-O_i) 
\Bigg\|_{V_t(\lambda)^{-1}}.$
Thus, we complete the proof of Proposition~\ref{prop:concentration}.
% \esmaeil{The problem with the above expression is that the sequence $\sum_{i=\ell(t)}^{t-1} \phi_i(a_i)\eta_i$ is not a martingale, so we cannot use Theorem 20.4 to bound it. I believe the sequence $\sum_{i=1}^{\ell(t)-1}\phi_i(a_i)\eta_i$ is a martingale adapted to the above filtration.}

% Let $\omega_i :=  \phi(s_j, a) \phi(s_j, a)^TO_i + 
% \bar{\phi}(a_i)\bar{\phi}(a_i)^T
% (1-O_i)$. Then 
% \begin{align*}
% (\tilde V_t(\lambda)^{-1}\tilde V_t &- V_t(\lambda)^{-1}V_t)(\tilde V_t-V_t)  \\
% &= \left({\left(\sum_{i=1}^{t-1}\omega_i\right)}{\left(\lambda I+\sum_{i=1}^{t-1}\omega_i\right)^{-1}} - {\left(\sum_{i=1}^{\ell(t)-1}\omega_i\right)}{\left(\lambda I+\sum_{i=1}^{\ell(t)-1}\omega_i\right)^{-1}}\right)\left(\sum_{i=\ell(t)}^{t-1}\omega_i\right)
% \\   
% &={\lambda \left(\sum_{i=\ell(t)}^{t-1}\omega_i\right)^2}{\left(\lambda I+\sum_{i=1}^{t-1}\omega_i\right)^{-1}\left(\lambda I+\sum_{i=1}^{\ell(t)-1}\omega_i\right)^{-1}}
% \\ & \leq
% {\lambda  \left(\sum_{i=\ell(t)}^{t-1}\omega_i\right)}{\left(\lambda I+\sum_{i=1}^{\ell(t)-1}\omega_i\right)^{-1}}
% \end{align*}
% \kyra{We note that $\sum_{i=\ell(t)}^{t-1}\omega_i$ is roughly $\prec \lambda I+\sum_{i=1}^{\ell(t)-1}\omega_i$ when $t-1-\ell(t)\leq \ell(t)-1$. That is when $t\leq 2\ell(t)$. Our robustness constraint ensures that $t\leq 4\ell(t)$. Can bound $ \left(\sum_{i=\ell(t)}^{t-1}\omega_i\right)\left(\lambda I+\sum_{i=1}^{\ell(t)-1}\omega_i\right)^{-1}$ with some constant times $I$ ??}
\end{proof}

\begin{prop}\label{thm:bandit_learning}
The Baysian regret of learning the contextual bandit in   Algorithm~\ref{alg:learning-reward} is bounded by $$\mathrm{BanditRegret}_T=\mathbb{E}\left[\sum_{t=1}^T \left\langle
    \phi_t(A_t^*) - \phi_t(\hat A_t) , \hat \theta (t)\right\rangle\right]\leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)}, $$ where $\beta = 1+\sqrt{2\log(T) +
d\log(1+\frac{TS^2L^2}{d})}
+ \|\sum_{i=\ell(t)}^{t-1}\phi_i\|_{V_t(\lambda)^{-1}}.$
\end{prop}
Now, we are ready to prove Theorem \ref{thm:bandit_learning}.
\begin{proof}[Proof of Proposition~\ref{thm:bandit_learning}] 
% At time $t$, let $\ell(t)$ denote the most recent time that we reveal $\mathcal{H}^{\mathrm{ir}}_{\ell(t)}$ to the treatment recommender.
Following the proof of Theorem 36.4 in \cite{lattimore2020bandit},
and letting $\phi_t(A_t) = \phi(S_t, A_t)O_t+\bar\phi(A_t)(1-O_t)$,
we define the upper confidence bound  function at time $t$:
    % when we reveal the context at time $t$:
$$U_{t}(\phi_{t}(A_{t}))  
= \left\langle
\phi_{t}(A_{t}), 
\tilde{\theta}_{t}\right\rangle 
+ \beta\left\|
\phi_{t}(A_{t})
\right\|_{V_{t}^{-1}},$$
with  
$V_{t} = 
% \lambda
\frac{1}{S^2}
I + \sum_{i=1}^{t-1} \phi_i(A_i) \phi_i(A_i)^T.
$

From Proposition~\ref{prop:concentration}, 
substitute $\lambda = 1/S^2$, and using the inequality that $\frac{\det{V_t(\lambda)}}{\lambda^d}\leq 
\left(\mathrm{trace}\left(\frac{V_t(\lambda)}{\lambda d}\right)\right)^d\leq \left(1+\frac{TL^2}{\lambda d}\right)^d$, 
we have that $\mathbb{P}\left(\exists t\leq T: \left\|\hat\theta_{t} - \theta\right\|_{V_t(\lambda)}>\beta
\right)\leq 1/T$, where 
$\beta = 1+\sqrt{2\log(T) +
d\log(1+\frac{TS^2L^2}{d})}
% \log\left(\frac{\det(\tilde V_t(\lambda))}{\lambda^q}\right)} + \sqrt{\lambda}\norm{\theta_*}_2 
+ \|\sum_{i=\ell(t)}^{t-1}\phi_i\|_{V_t(\lambda)^{-1}}$. 
% To bound the last term, following Lemma 19.4 of \cite{lattimore2020bandit}, we have
% \begin{align*} \left\|\sum_{i=\ell(t)}^{t-1}\phi_i\right\|^2_{V_t(\lambda)^{-1}} 
% &\leq \sum_{i=\ell(t)}^{t-1}\left\|\phi_i\right\|^2_{V_t(\lambda)^{-1}} 
% \leq  \sum_{i=\ell(t)}^{t-1}\min\left(1,
% \left\|\phi_i\right\|^2_{V_t(\lambda)^{-1}}\right)\leq 2\sum_{i=\ell(t)}^{t-1}
% \log\left(1 + \left\|\phi_i\right\|_{V_t(\lambda)^{-1}}^2 \right) \\
% &\leq 2\log\left(\frac{\det V_{t-1}}{\det V_{\ell(t)-1}}\right)
% \end{align*}
% \kyra{We can loosely bound the above term by $\det V_{t-1}/\det V_0$, not sure whether we can get anything tighter.} 

Let $E_t$ be the event that $\left|\langle\tilde\theta_t -  \theta, \phi_t(A_t)\rangle\right|\leq \beta$, and $E = \bigcap_{t=1}^T E_t$. Let $A^*_t = \argmax_{a\in \mathcal{A}}\langle\phi(S_t,a)O_t+\bar\phi(a)(1-O_t),\theta\rangle$. 
% and let $\phi_t = \phi(s_t, a)\mathbbm{1}_{O_t=1}+\bar\phi(a)\mathbbm{1}_{O_t\neq 1}$. 
We note here that $A_t^*$ is a random variable since $\theta$ is random. In addition, $A_t^*$ depends on the $S_t$ and $O_t$. 
Let $\hat A_t = \argmax_{a\in \mathcal{A}}\langle\hat \theta_t, \phi_t(a)\rangle$, and let $\tilde A_t = \argmax_{a\in\mathcal{A}}\langle\tilde\theta_t, \phi_t(a)\rangle$.
Thus, the regret at time $t$ is
\begin{align*}
&\mathrm{BanditRegret}_T =
\mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(\hat A_t), \hat\theta(t) \right\rangle\right]\\&
    = \mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(\tilde A_t) +  \phi_t(\tilde A_t) - \phi_t(\hat A_t) , \hat \theta(t)\right\rangle\right]
    \\&
    = \mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(\tilde A_t), \hat\theta(t)\right\rangle\right] +  \mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle\phi_t(\tilde A_t) - \phi_t(\hat A_t) , \hat\theta(t) \right\rangle\right],
    \\&
=\mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(\tilde A_t), \hat\theta(t)\right\rangle\right] +  \mathbb{E}_{\theta, O}\left[\sum_{t=1}^T \left\langle\phi_t(\tilde A_t) - \phi_t(\hat A_t) , 
    \hat \theta(t) \right\rangle \mathbbm{1}_{\tilde A_t \neq \hat A_t, O_t=0}\right].
    \end{align*}
The first term is the standard Bayesian bandit loss where we observe the entire history up to time $t$. The second term is obtained due to the fact that  when $O_t=1$, $\tilde\theta(t) = \hat\theta(t)$ and $\tilde A_t = \hat A_t$.
% For the information revealer, let $\mathcal{F}_{t}=\sigma\left(X_1, ..., X_{t-1}, \phi_1(A_1), ..., \phi_{t}(A_{t}) \right)$ be the $\sigma$-algebra.
% Let $\mathbb{E}_{t}[\cdot] = \mathbb{E}[\cdot|\mathcal{F}_{t}]$. Note that the definition of Thompson sampling implies that the conditional distribution of $\phi_t(A_t^*)$ and $\phi_t(A_t)$ given $\mathcal{F}_{t}$ are the same: $\mathbb{P}(\phi_t(A_t^*)=\cdot|\mathcal{F}_{t}) = \mathbb{P}(\phi_t(A_t) = \cdot|\mathcal{F}_t)$ a.s. Furthermore, $U_t(\phi_t(a))$ is $\mathcal{F}_t$-measurable for any fixed $a\in\mathcal{A}$. Thus, we have that $\mathbb{E}_t[U_t(\phi_t(A^*_t))] = \mathbb{E}_t[U_t(\phi_t(A_t))]$.
Thus, we can bound the second term above 
\begin{align*}
    \mathbb{E}_{\theta, O} &\left[ \left\langle\phi_t(\tilde A_t) - \phi_t(\hat A_t) , \theta \right\rangle \mathbbm{1}_{\tilde A_t \neq \hat A_t, O_t=0}\right]
    =\mathbbm{1}_{O_t=0}  \mathbbm{1}_{\tilde A_t \neq \hat A_t}\mathbb{E}_{t,\theta}\left[ \left\langle\bar\phi(\tilde A_t) - \bar\phi(\hat A_t) , \theta \right\rangle \right]
    \\&
    = (1-o_t)\mathbbm{1}_{\tilde A_t \neq \hat A_t}
    % \mathbb{E}_{t,\theta}\left[ \left\langle
    % \bar\phi(\tilde A_t) , \theta \right\rangle- 
    % U_t(\bar\phi_t(\tilde A_t)) +
    % U_t(\bar\phi_t(\tilde A_t)) -
    % \left\langle
    % \bar\phi(\hat A_t) , \theta \right\rangle \right]\\&
    % \leq (1-o_t)\mathbbm{1}_{\tilde A_t \neq \hat A_t}\mathbb{E}_{t,\theta}\left[ 
    % U_t(\bar\phi_t(\tilde A_t)) -\left\langle
    % \bar\phi(\hat A_t) , \theta \right\rangle \right]
\end{align*}
    
    \begin{align*}
    \mathrm{BanditRegret}_T &
=\mathbb{E}\left[\mathbbm{1}_{E^c} \sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(a_t) , \theta \right\rangle\right] + \mathbb{E}\left[\mathbbm{1}_{E}\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(a_t) , \theta \right\rangle\right]\\
    &\leq 2+\mathbb{E}\left[\mathbbm{1}_{E}\sum_{t=1}^T \left\langle
    \phi_t(A^*_t) - \phi_t(a_t) , \theta \right\rangle\right]
    \\&
    \leq 2+ \mathbb{E}\left[\sum_{t=1}^T \mathbbm{1}_{E_t}\left\langle
    \phi_t(A^*_t) - \phi_t(a_t) , \theta \right\rangle\right].
\end{align*}
Let $\mathcal{F}_{t}=\sigma\left(X_1, ..., X_{\ell(t)-1}, \phi_1(A_1), ..., \phi_{\ell(t)}(A_{\ell(t)}) \right)$ and let $\mathbb{E}_{t}[\cdot] = \mathbb{E}[\cdot|\mathcal{F}_{t}]$. Note that the definition of Thompson sampling implies that the conditional distribution of $\phi^*$ and $\phi_t$ given $\mathcal{F}_{t}$ are the same: $\mathbb{P}(\phi^*=\cdot|\mathcal{F}_{t}) = \mathbb{P}(\phi_t = \cdot|\mathcal{F}_t)$ a.s. Furthermore, $U_t(\phi_t)$ is $\mathcal{F}_t$-measurable for any fixed $a\in\mathcal{A}$. Thus, we have that $\mathbb{E}_t[U_t(\phi^*)] = \mathbb{E}_t[U_t(\phi_t)]$. Thus, we can bound the second term above 
\begin{align*}
\mathbb{E}\left[\mathbbm{1}_{E_t}\left\langle
    \phi^* - \phi_t , \theta \right\rangle\right]&= \mathbbm{1}_{E_t}\mathbb{E}_{t}\left[\langle\phi^*,\theta\rangle - U_t(\phi^*) + U_t(\phi_t) -\langle\phi_t, \theta\rangle\right]\\
    &\leq 
    \mathbbm{1}_{E_t}\mathbb{E}_{t}\left[U_t(\phi_t) -\langle\phi_t, \theta\rangle\right]\\
   & \leq \mathbbm{1}_{E_t}\mathbb{E}_{t}\left[\langle\phi_t,\hat\theta_t - \theta\rangle\right] + \beta \|\phi_t\|_{V_t^{-1}}\\
   &\leq \mathbbm{1}_{E_t}\mathbb{E}_{t}\left[\|\phi_t\|_{V_t^{-1}}\|\hat\theta_t - \theta\|_{V_t^{-1}}\right] + \beta \|\phi_t\|_{V_t^{-1}}\\
   &\leq 2\beta\|\phi_t\|_{V_t^{-1}}.
\end{align*}
Thus, by Cauchy-Schwarz we have
\begin{align*}
\mathbb{E}\left[\sum_{t=1}^T \mathbbm{1}_{E_t}\left\langle\phi^* - \phi_t , \theta \right\rangle\right] 
&\leq 2\beta \mathbb{E}\left[\sum_{t=1}^T\min \left(1, \|\phi_t\|_{V_t^{-1}}\right)\right]\\
&\leq 2\sqrt{T\beta^2\mathbb{E}\left[\sum_{t=1}^T\min \left(1, \|\phi_t\|^2_{V_t^{-1}}\right)\right]}\\
&\leq 2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)},
\end{align*}
where the last inequality follows from Lemma 19.4 of \cite{lattimore2020bandit}.

Together, we obtain that $$\mathbb{E}\left[\sum_{t=1}^T \left\langle
    \phi^* - \phi_t , \theta \right\rangle\right]\leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)},$$ where $\beta = $
\end{proof}


\begin{thm}\label{thm:mainresult}
The Baysian regret of Algorithm~\ref{alg:learning-reward} is bounded as follows: 
\begin{align*}
\mathrm{BayesianRegret} \leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)} + \left( 1 - \alpha \right)  
\mathbb{E}\left[ V^{\text{Oracle}} \right],
\end{align*}
where $\alpha = \left(1+\frac{1}{c-1}\right)\frac{1}{\eta_{\min}}$.
\end{thm}

\begin{proof}[Proof of Theorem~\ref{thm:bandit_learning}] 
Recall we defined three models and then established the following bridging argument for the regret decomposition:
\begin{align*}
\text{BayesianRegret} & = \mathbb{E}\left[ V^{\text{Oracle}} \right] - \mathbb{E}\left[ V^{\text{ALG}} \right] \\
& = \underbrace{ \mathbb{E}\left[ V^{\text{Auxiliary}} - V^{\text{ALG}} \right] }_\text{contextual bandit loss} + \underbrace{ \mathbb{E}\left[ V^{\text{Oracle}} - V^{\text{Auxiliary}} \right] }_\text{allocation decision loss}.
\end{align*}

From our primal-dual analysis, we derive the following competitive ratio:
$$
V^{\text{Auxiliary}} / V^{\text{Oracle}}
\geq \left(1+\frac{1}{c-1}\right)\frac{1}{\eta_{\min}},
$$
which implies the following by a simple algebra and letting $\alpha = \left(1+\frac{1}{c-1}\right)\frac{1}{\eta_{\min}}$:
$$
 V^{\text{Oracle}} - V^{\text{Auxiliary}} \leq 
 \left( 1 - \alpha \right) V^{\text{Oracle}}.
$$
Next, taking an expectation over the prior distribution of the unknown parameter $\theta$ on both sides, we can obtain the following:
$$
\mathbb{E}\left[ V^{\text{Oracle}} - V^{\text{Auxiliary}} \right]
\leq 
\left( 1 - \alpha \right)  
\mathbb{E}\left[ V^{\text{Oracle}} \right].
$$
Also, from our Theorem \ref{thm:bandit_learning}, we have the following:
$$
\mathbb{E}\left[ V^{\text{Auxiliary}} - V^{\text{ALG}} \right]
\leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)}.
$$
So, summing the upper bounds established above for each term, we have the following:
\begin{align*}
\text{BayesianRegret} \leq 2+2\sqrt{2dT\beta^2\log\left(1+\frac{TS^2L^2}{d}\right)} + \left( 1 - \alpha \right)  
\mathbb{E}\left[ V^{\text{Oracle}} \right].
\end{align*}
\end{proof}

